Kinematic properties of the dual AGN system J0038+4128 based on long-slit spectroscopy

The study of kiloparsec-scale dual active galactic nuclei (AGN) will provide important clues to understand the co-evolution between the host galaxies and their central supermassive black holes undergoing a merging process. We present long-slit spectroscopy of the J0038$+$4128, a kiloparsec-scale dual AGN candidate discovered by Huang et al. recently, using the Yunnan Faint Object Spectrograph and Camera (YFOSC) mounted on Li-Jiang 2.4-m telescope at Yunnan observatories. From the long-slit spectra, we find that the average relative line-of-sight (LOS) velocity between the two nuclei (J0038$+$4128N and J0038$+$4128S) is about 150 km s$^{-1}$. The LOS velocities of the emission lines from the gas ionized by the nuclei activities and of the absorption lines from stars governed by the host galaxies for different regions of the J0038$+$4128 exhibit the same trend. The same velocities trend indicates that the gaseous disks are co-rotating with the stellar disks in this ongoing merge system. We also find several knots/giant HII regions scattered around the two nuclei with strong star formation revealed by the observed line ratios from the spectra. Those regions are also detected clearly in HST $F336W/U$-band and HST $F555W/V$-band images.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

